Ensembled Prediction Intervals for Causal Outcomes Under Hidden Confounding

Causal inference of exact individual treatment outcomes in the presence of hidden confounders is rarely possible. Recent work has extended prediction intervals with finite-sample guarantees to partially identifiable causal outcomes, by means of a sensitivity model for hidden confounding. In deep learning, predictors can exploit their inductive biases for better generalization out of sample. We argue that the structure inherent to a deep ensemble should inform a tighter partial identification of the causal outcomes that they predict. We therefore introduce an approach termed Caus-Modens, for characterizing causal outcome intervals by modulated ensembles. We present a simple approach to partial identification using existing causal sensitivity models and show empirically that Caus-Modens gives tighter outcome intervals, as measured by the necessary interval size to achieve sufficient coverage. The last of our three diverse benchmarks is a novel usage of GPT-4 for observational experiments with unknown but probeable ground truth.

==> benchmark-aita.tex <==
\subsection{Novel Benchmark on GPT-3.5 \texttt{(AITA)}}\label{sec:bench-aita}
Semi-synthetic causal benchmarks like \texttt{PBMC} can be designed to harness the arbitrary statistical relations in real data. Still, the outcome link must take on a specific functional form---modulo the treatment and all confounders. In our desire to limit the influence of design choices on the experimental validity, we constructed a new causal benchmark via the large language model GPT-3.5~\citep{brown20}. Such a flexible generative model is capable of emulating nontrivial dynamics in text. Crucially, the practice of prompting makes it possible to query \emph{interventions} and directly measure causal effects. We propose a dataset in our final experiment and seek to promote this usage of large generative models for benchmarking in causal inference~\citep{curth}.

We framed the novel inference task in the format of the well-known subreddit r/AmITheAsshole (hence the name, \texttt{AITA}.) This subreddit has recently served as a vessel for data on human perspectives~\citep{botzer22} and moral judgment~\citep{plepi22} in the computational social sciences. It is a scientifically attractive setting because the rules and structure of the forum are clean: users post personal stories of conflict, and comments offer opinions on whether the poster was at fault in the way the story transpired. A verdict can be considered the top-voted comment, or all comments weighted by their upvotes. As GPT-3.5 is familiar with subreddits, having it focus on a known context simplifies the engineering of prompts. Furthermore, since handling real data introduces considerations that are out of the scope of our experiments, we opted for completely synthetic r/AmITheAsshole posts \emph{and} verdicts. In one session, we would ask GPT-3.5 to generate a post, a list of associated topic keywords, and a list of moral valences. Those lists served as covariates. Hidden confounding was considered the relevant information contained in the posts beyond the provided topics and morals. In another session, we would ask the language model to give a simple YTA/NTA (``you're the asshole'' vs.\ ``not the asshole'') verdict for a synthetic post, 32 separate times. The ratio of YTA to NTA allowed the estimation of logits that served as the outcome. Finally, the treatment variable was considered to be the binary sex of the synthetic poster. All generated posts began with statements like ``I~(23F)~\dots'' marking the protagonist's age and binary sex, as is customary in the real subreddit. This (rather limited) form of self-identification permitted causal experimentation with binary treatments and the typical MSM. To simulate interventions, we would swap the M/F letter in that identifier and re-estimate the outcome logits by querying GPT-3.5 again.

\begin{figure}[!ht]
  \vspace{-0.5em}
  \begin{minipage}{0.45\linewidth}
    \scalebox{0.80}{
      \input{figures/aita-hist.pgf}}
  \end{minipage}
  \hfill
  \begin{minipage}{0.52\linewidth}
    \scalebox{0.80}{
      \input{figures/aita-hist-2.pgf}}
  \end{minipage}\vspace{-0.75em}
  \caption{\label{fig:aita-analysis}Relevant statistics of the proposed \texttt{AITA} dataset. \textbf{Left}: histogram of the entire 1,024-size sample of outcomes, right-shifted to be all positive. The heavy right-skew of this variable motivated the decision to model the outcome predictions as exponentially distributed. \textbf{Right}: visualizing the counterfactuals in the 256-size test set. Upper plot shows cumulative frequencies of the potential outcomes; lower plot shows the realized ITEs of M $\to$ F. Clearly, there is a negative causal effect.}
\end{figure}

\paragraph{Covariate dimensionality reduction.}
The entire post, sans the treatment identifier, comprised the whole set of possible confounders that could influence GPT-3.5's verdict. As mentioned above, the topic and moral-valence keywords were chosen as the observable portion of the confounders. We employed a pretrained Roberta sentence transformer~\citep{liu19} to embed the keyword lists and obtain pairwise cosine similarities between posts. Then, once for topics and once for moral valences, we computed the three major eigenvectors of the normalized graph Laplacians in a similar manner to diffusion maps~\citep{nadler05}. This way, we obtained six real-valued covariates per post that represented its distinctive topic and moral-valence information.

\paragraph{Preliminary analysis.}
We \emph{i.i.d} sampled a training set of 512 posts, validation set of 256, and test set of 256. The data were unbalanced: 76\% of posts were assigned treatment F(emale) and the other 24\% were assigned M(ale). We were not concerned by this phenomenon because the causal methodology is supposed to address the domain shift between biased observational data and a randomized causal setting. Another imbalance in the dataset was the generative model's tendency to favor not blaming the protagonist of the post. As evidenced in Figure~\ref{fig:aita-analysis} (left), the NTA -- YTA outcomes greatly leaned leftward. This persisted even after light tweaking of the prompt to eschew the derogatory language inherent in the NTA/YTA verdict system. As shown in Figure~\ref{fig:aita-analysis}, we shifted the outcome distribution and hence modeled the conditional outcomes with an exponential distribution. In this particular benchmark the outcome intervals were right sided, using $[0, F^{-1}(1-\alpha)]$ rather than the central version $[F^{-1}(\alpha/2), F^{-1}(1-\alpha/2)]$ that was employed in all other experiments. Coverage was quantified on the male arm of the test-set potential outcomes, since that arm was much less observed. %in the empirical distribution.

It is critical for a discernible causal effect to really exist in the system. As shown in Figure~\ref{fig:aita-analysis} (right), there clearly was. Indeed, the average treatment effect (ATE) estimated on the test set for {M $\to$ F} was $-0.76$ ($-1.37$ median), 11\% (20\%) of the total range, with a Wilcoxon signed-rank $p < 10^{-10}$.


\paragraph{Cost function.}
As mentioned above, the emulated verdict outcomes were quantified on a heavily skewed logit spectrum. Even though they were bounded on both sides, their frequencies called for an exponential approximation with support on the nonnegative reals. The cost function took into account their bounded nature by taking the causal interval length as a percentage of the entire support interval and ceiling at 100\% prior to averaging different trials.


\begin{table}[!ht]\centering 
  \begin{tabular}{l l | r r }
    Target Coverage & Method & Achieved Coverage $\uparrow$ & Efficiency Cost $\downarrow$ \\
    \midrule
    90\% & Caus-Modens & 87.7 (2.1) \% & \textbf{59.1} (1.1) \% \\
     & Ens-CSA-DCP & \textbf{96.6} (2.1) \% & 79.1 (7.6) \% \\
     & Ens-CSA-CQR & \textbf{95.3} (2.5) \% & 73.1 (7.7) \% \\
     & CSA-DCP & \textbf{96.6} (2.6) \% & 80.9 (9.8) \% \\
     & Ens-DCP & \textbf{96.6} (1.8) \% & 77.3 (4.2) \% \\
    \midrule
    95\% & Caus-Modens & \textbf{96.3} (1.1) \% & \textbf{75.4} (2.2) \% \\
     & Ens-CSA-DCP & \textbf{98.7} (1.3) \% & 90.4 (7.2) \% \\
     & Ens-CSA-CQR & \textbf{98.5} (1.3) \% & 87.4 (9.1) \% \\
     & CSA-DCP & \textbf{98.9} (1.3) \% & 91.5 (7.3) \% \\
     & Ens-DCP & \textbf{98.9} (0.9) \% & 90.7 (4.7) \% \\
    \midrule
    99\% & Caus-Modens & \textbf{99.8} (0.3) \% & \textbf{95.7} (2.9) \% \\
    & Ens-CSA-DCP & \textbf{99.9} (0.3) \% & 98.7 (2.8) \% \\
    & Ens-CSA-CQR & \textbf{100.0} (0.1) \% & 99.0 (2.3) \% \\
    & CSA-DCP & \textbf{100.0} (0.2) \% & 98.7 (2.3) \% \\
    & Ens-DCP & \textbf{100.0} (0.0) \% & 99.8 (0.4) \% \\
  \end{tabular}\vspace{0.50em}

  \caption{\label{tab:aita}Means (\& standard deviations) of achieved coverages and costs thereof for the \texttt{AITA} benchmark with ensembles of size 64. Data and predictors were bootstrap resampled for the scatter estimates. The efficiency cost is expressed as a percentage of the outcome range. For achieved coverage, all valid results are in bold. For efficiency cost, the lowest in each group is bold.}
\end{table}


\paragraph{Results.}
We performed an extensive ablation study on the novel \texttt{AITA} dataset and present the results in Table~\ref{tab:aita}. We listed two quantities of interest to measure a method's efficacy: the achieved coverage, which should be greater than the target coverage, and the efficiency cost, which should be as low as possible. The expression of the cost as a percentage in this experiment makes it more interpretable for viewing causal predictions in terms of actionability. For instance, the efficiency cost of Caus-Modens at $\sim$90\% coverage is $\sim$60\%, so a significant portion ($\sim$40\% on average) of the outcome spectrum is ruled out by the Caus-Modens outcome intervals on posts in the test set. Therefore, the de-confounded verdict predictions carry some information about the GPT-3.5 outcomes while maintaining coverage, unlike those settings where the efficiency cost approaches 100\%.
